Logarithmically slow domain growth in nonrandomly frustrated systems: Ising models with competing interactions

It is known that in systems which contain randomness explicitly in their Hamiltonians (e.g., due to impurities), the characteristic size L of the ordered domains can grow only logarithmically with time t following a quench below the transition temperature. However, in systems without such imposed randomness, much faster power law growth has generally been predicted. Motivated by the slow dynamics present in glasses, we have been looking for counterexamples, i.e., for models without randomness which nonetheless order logarithmically slowly. Here, we discuss two closely related models for which we have simple physical arguments that such slow growth occurs. The basis of these arguments is the claim that the free energy barriers to domain growth in these models are proportional to L. Thus, the barriers grow as the domains coarsen. We present the results of Monte Carlo simulations, which lend strong support to our claims of growing barriers and logarithmically slow dynamics. Finally, we discuss how quickly the system orders when it is cooled continuously through the transition (rather than quenched).

==> 9204015.2 <==
%%  9204015 (part 3)

%%%%%%%%%%%%%%%%%%%%jnl_shore.tex%%%%%%%%%%%%%%%%%%%%%%%%%%

%	JNL.TEX					Doug Eardley
%      Modified by Joel Shore

\font\twelverm=amr10 scaled 1200    \font\twelvei=ammi10 scaled 1200
\font\twelvesy=amsy10 scaled 1200   \font\twelveex=amex10 scaled 1200
\font\twelvebf=ambx10 scaled 1200   \font\twelvesl=amsl10 scaled 1200
\font\twelvett=amtt10 scaled 1200   \font\twelveit=amti10 scaled 1200

\skewchar\twelvei='177   \skewchar\twelvesy='60

\def\twelvepoint{\normalbaselineskip=12.4pt plus 0.1pt minus 0.1pt
  \abovedisplayskip 12.4pt plus 3pt minus 9pt
  \belowdisplayskip 12.4pt plus 3pt minus 9pt
  \abovedisplayshortskip 0pt plus 3pt
  \belowdisplayshortskip 7.2pt plus 3pt minus 4pt
  \smallskipamount=3.6pt plus1.2pt minus1.2pt
  \medskipamount=7.2pt plus2.4pt minus2.4pt
  \bigskipamount=14.4pt plus4.8pt minus4.8pt
  \def\rm{\fam0\twelverm}          \def\it{\fam\itfam\twelveit}%
  \def\sl{\fam\slfam\twelvesl}     \def\bf{\fam\bffam\twelvebf}%
  \def\mit{\fam 1}                 \def\cal{\fam 2}%
  \def\tt{\twelvett}
  \textfont0=\twelverm   \scriptfont0=\tenrm   \scriptscriptfont0=\sevenrm
  \textfont1=\twelvei    \scriptfont1=\teni    \scriptscriptfont1=\seveni
  \textfont2=\twelvesy   \scriptfont2=\tensy   \scriptscriptfont2=\sevensy
  \textfont3=\twelveex   \scriptfont3=\twelveex  \scriptscriptfont3=\twelveex
  \textfont\itfam=\twelveit
  \textfont\slfam=\twelvesl
  \textfont\bffam=\twelvebf \scriptfont\bffam=\tenbf
  \scriptscriptfont\bffam=\sevenbf
  \normalbaselines\rm}

\def\tenpoint{\normalbaselineskip=12pt plus 0.1pt minus 0.1pt
  \abovedisplayskip 12pt plus 3pt minus 9pt
  \belowdisplayskip 12pt plus 3pt minus 9pt
  \abovedisplayshortskip 0pt plus 3pt
  \belowdisplayshortskip 7pt plus 3pt minus 4pt
  \smallskipamount=3pt plus1pt minus1pt
  \medskipamount=6pt plus2pt minus2pt
  \bigskipamount=12pt plus4pt minus4pt
  \def\rm{\fam0\tenrm}          \def\it{\fam\itfam\tenit}%
  \def\sl{\fam\slfam\tensl}     \def\bf{\fam\bffam\tenbf}%
  \def\smc{\tensmc}             \def\mit{\fam 1}%
  \def\cal{\fam 2}%
  \textfont0=\tenrm   \scriptfont0=\sevenrm   \scriptscriptfont0=\fiverm
  \textfont1=\teni    \scriptfont1=\seveni    \scriptscriptfont1=\fivei
  \textfont2=\tensy   \scriptfont2=\sevensy   \scriptscriptfont2=\fivesy
  \textfont3=\tenex   \scriptfont3=\tenex     \scriptscriptfont3=\tenex
  \textfont\itfam=\tenit
  \textfont\slfam=\tensl
  \textfont\bffam=\tenbf \scriptfont\bffam=\sevenbf
  \scriptscriptfont\bffam=\fivebf
  \normalbaselines\rm}

\let\bigtype=\twelvepoint
\let\medtype=\tenpoint

\def\beginlinemode{\endmode
  \begingroup\parskip=0pt \obeylines\def\\{\par}\def\endmode{\par\endgroup}}
\def\beginparmode{\endmode
  \begingroup \def\endmode{\par\endgroup}}
\let\endmode=\par
{\obeylines\gdef\
{}}
\def\singlespace{\baselineskip=\normalbaselineskip}
\def\oneandathirdspace{\baselineskip=\normalbaselineskip
  \multiply\baselineskip by 4 \divide\baselineskip by 3}
\def\oneandahalfspace{\baselineskip=\normalbaselineskip
  \multiply\baselineskip by 3 \divide\baselineskip by 2}
\def\doublespace{\baselineskip=\normalbaselineskip \multiply\baselineskip by 2}
\def\triplespace{\baselineskip=\normalbaselineskip \multiply\baselineskip by 3}
\newcount\firstpageno
\firstpageno=2
\footline={\ifnum\pageno<\firstpageno{\hfil}
	\else{\hfil\twelverm\folio\hfil}\fi}
\def\toppageno{\global\footline={\hfil}\global\headline
  ={\ifnum\pageno<\firstpageno{\hfil}\else{\hfil\twelverm\folio\hfil}\fi}}
\def\nopageno{\global\footline={\hfil}}
\let\rawfootnote=\footnote		% We must set the footnote style
\def\footnote#1#2{{\rm\singlespace\parindent=0.17truein\parskip=0pt
  \rawfootnote{#1}{#2\hfill\vrule height 0pt depth 6pt width 0pt}}}
%\def\footnote#1#2{{\rm\singlespace\parindent=0pt\parskip=0pt
%  \rawfootnote{#1}{#2\hfill\vrule height 0pt depth 6pt width 0pt}}}
\def\raggedcenter{\leftskip=4em plus 12em \rightskip=\leftskip
  \parindent=0pt \parfillskip=0pt \spaceskip=.3333em \xspaceskip=.5em
  \pretolerance=9999 \tolerance=9999
  \hyphenpenalty=9999 \exhyphenpenalty=9999 }
\def\dateline{\rightline{\ifcase\month\or
  January\or February\or March\or April\or May\or June\or
  July\or August\or September\or October\or November\or December\fi
  \space\number\year}}
\def\today{\ifcase\month\or
  January\or February\or March\or April\or May\or June\or
  July\or August\or September\or October\or November\or December\fi
  \space\number\day, \number\year}
\def\received{\vskip 3pt plus 0.2fill
 \centerline{\sl (Received\space\ifcase\month\or
  January\or February\or March\or April\or May\or June\or
  July\or August\or September\or October\or November\or December\fi
  \qquad, \number\year)}}

\hsize=6.5truein
\hoffset=0truein
\vsize=8.9truein
\voffset=0truein
\parskip=\medskipamount
\def\\{\cr}
\twelvepoint		% selects twelvepoint fonts (cf. \tenpoint)
\oneandahalfspace	% selects double spacing for main part of paper (cf.
			%	\singlespace, \oneandahalfspace)
\overfullrule=0pt	% delete the nasty little black boxes for overfull box


\def\draft
  {\noindent {\bf DRAFT: \today}\hfill\break}

\def\nsfitp#1{
 \rightline{\rm NSF--ITP--#1}}	% Preprint number at upper right of title page

\def\title			%  Title on title page
  {\null\vskip 3pt plus 0.2fill
   \beginlinemode \doublespace \raggedcenter \bf}

\def\author			%  Author(s) name(s)  on title page
  {\vskip 3pt plus 0.2fill \beginlinemode
   \singlespace \raggedcenter}

\def\affil			% Affiliations (can intermix with \author)
  {\vskip 3pt plus 0.1fill \beginlinemode
   \oneandahalfspace \raggedcenter \sl}

\def\abstract			% Begin abstract
  {\vskip 3pt plus 0.3fill \beginparmode
   \oneandahalfspace ABSTRACT: }

\def\submit  			% submission journal statement
	{\vskip 24pt \beginlinemode
	\noindent \rm Submitted to: \sl}

\def\endtopmatter		% End title page, begin body of paper
  {\endpage			% 	This subsumes \body
   \body}

\def\body			% Begin text body;  can be used to end
  {\beginparmode}		% \title, \author, \affil, \abstract,
				% \reference, or \figurecaption modes

\def\head#1{			% Head;  NOTE enclose the text in {}
  \goodbreak\vskip 0.5truein	%  e.g., \head{I. Introduction}
  {\immediate\write16{#1}
   \raggedcenter \uppercase{#1}\par}
   \nobreak\vskip 0.25truein\nobreak}

\def\subhead#1{			% Subhead;  NOTE enclose the text in {}
  \vskip 0.25truein		% e.g., \subhead{A. History of the Problem}
  {\raggedcenter #1 \par}
   \nobreak\vskip 0.25truein\nobreak}

\def\beneathrel#1\under#2{\mathrel{\mathop{#2}\limits_{#1}}}

\def\refto#1{$^{#1}$}		% For references in text as superscript

\def\references			% Begin references -- basic format is Phys Rev
  {
%  \head{References}		% I.e., volume, page, year (space after commas).
   \beginparmode
   \singlespace
%  \doublespace
   \frenchspacing \parindent=0pt \leftskip=1truecm
   \parskip=8pt plus 3pt \everypar{\hangindent=\parindent}}

\gdef\refis#1{\item{#1.\ }}			% Ref list numbers.

\gdef\journal#1, #2, #3, 1#4#5#6{		% Journal reference.  Comma sets
    {\sl #1~}{\bf #2}, #3 (1#4#5#6)}		% off: name, vol, page, year

\def\refstylenp{		% Nucl Phys(or Phys Lett) ref style: V, Y, P
  \gdef\refto##1{ [##1]}			% Reference in text []
  \gdef\refis##1{\item{##1)\ }}			% Reference list numbers)
  \gdef\journal##1, ##2, ##3, ##4 {		% Journal reference
     {\sl ##1~}{\bf ##2~}(##3) ##4 }}

\def\refstyleprnp{		% Input like pr, output like np!!
  \gdef\refto##1{ [##1]}			% Reference in text []
  \gdef\refis##1{\item{##1)\ }}			% Reference list numbers)
  \gdef\journal##1, ##2, ##3, 1##4##5##6{	% Journal reference
    {\sl ##1~}{\bf ##2~}(1##4##5##6) ##3}}

\def\pr{\journal Phys. Rev., }

\def\pra{\journal Phys. Rev. A, }

\def\prb{\journal Phys. Rev. B, }

\def\prc{\journal Phys. Rev. C, }

\def\prd{\journal Phys. Rev. D, }

\def\prl{\journal Phys. Rev. Lett., }

\def\jmp{\journal J. Math. Phys., }

\def\rmp{\journal Rev. Mod. Phys., }

\def\cmp{\journal Comm. Math. Phys., }

\def\np{\journal Nucl. Phys., }

\def\pl{\journal Phys. Lett., }

\def\apj{\journal Astrophys. Jour., }

\def\apjl{\journal Astrophys. Jour. Lett., }

\def\annp{\journal Ann. Phys. (N.Y.), }

\def\endreferences{\body}

\def\figurecaptions		% Begin figure captions
  {\endpage
   \beginparmode
   \head{Figure Captions}
   \singlespace
%  \doublespace
%  \parskip=24pt plus 3pt \everypar={\hangindent=4em}
}

\def\endfigurecaptions{\body}

\def\endpage			%  Eject a page
  {\vfill\eject}

\def\endpaper			%  Ways to say goodbye
  {\endmode\vfill\supereject}
\def\endjnl
  {\endpaper}
\def\endit
  {\endpaper\end}

\def\ref#1{Ref.~#1}                     %       for inline references
\def\Ref#1{Ref.~#1}                     %       ditto
\def\[#1]{[\cite{#1}]}
\def\cite#1{{#1}}
\def\(#1){(\call{#1})}
\def\call#1{{#1}}
\def\taghead#1{}
\def\frac#1#2{{#1 \over #2}}
\def\half{{\frac 12}}
\def\third{{\frac 13}}
\def\fourth{{\frac 14}}
\def\12{{1\over2}}
\def\eg{{\it e.g.,\ }}
\def\Eg{{\it E.g.,\ }}
\def\ie{{\it i.e.,\ }}
\def\Ie{{\it I.e.,\ }}
\def\etal{{\it et al.\ }}
\def\etc{{\it etc.\ }}

%A set of definitions which supplements the ``standard'' jnl
%definitions.

\font\titlefont=ambx10 scaled \magstep3  %Use very big font for chapter title
\font\sectionfont=ambx10 scaled \magstep2  %Use big font for section but
                                           %not subsection

%Define some partial derivatives.
\def\pd#1#2{{\frac{\partial #1}{\partial #2}}}
\def\ppd#1#2{{\frac{{\partial}^2 #1}{\partial {#2}^2}}}
\def\der#1#2{{\frac{d #1}{d #2}}}
\def\dder#1#2{{\frac{d^2 #1}{d {#2}^2}}}
%Miscellaneous
%Some journal definitions.
\def\surf{\journal Surf. Sci., }
\def\pscripta{\journal Physica Scripta, }
\def\jdp{\journal J. Phys. (Paris), }
\def\ssc{\journal Solid State Comm., }
%LASSP affiliation.
\def\lassp{Laboratory of Atomic and Solid State Physics\\Cornell
     University\\Ithaca, New York 14853-2501}
%PACS line on first page.
\def\pacs{\vskip 3pt plus 0.2fill \noindent  PACS numbers: }

%--- Homegrown math macros
% approximately greater than
\def\simgt{\mathrel{\lower .3ex \rlap{$\sim$}\raise .5ex \hbox{$>$}}}
%
% approximately less than
\def\simlt{\mathrel{\lower .3ex \rlap{$\sim$}\raise .5ex \hbox{$<$}}}
%
% Trace.
\def\Tr{{\mathop{\rm Tr}}}
%
% <bra|, |ket>, and <bra|ket>
\def\bra<#1|{\left\langle #1 \right|}
\def\ket|#1>{\left| #1 \right\rangle}
\def\braket<#1|#2>{\langle#1 | #2 \rangle}
%
\def\Int{\int\limits}			% Integral sign with sensible limits.
\def\Real{{\mathop{\rm Re}}}		% Readable real.
\def\ddt#1{{d#1\over dt}}		% derivative wrt t
\def\ddx#1{{d#1\over dx}}		% derivative wrt x
\def\ddxp#1#2{{\partial #2\over\partial #1}}
\def\dop#1{{\partial\over\partial #1}}
\def\dsq#1{{\partial^2\over\partial {#1}^2}}
\def\dmix#1#2{{\partial^2\over\partial #1\partial #2}}
\def\Dmix#1#2#3{{\partial^2 #3 \over\partial #1\partial #2}}

\def\eqtitle#1{\par #1 \vskip -56pt}
\def\eqaligntitle#1{\par #1 \vskip -68pt}

\def\bull{\vrule height .9ex width .8ex depth -.1ex}					% Square bullet

% For including figures for dvi2ps.
\input psfig
\def\boxit#1{\vbox{\hrule\hbox{\vrule\vbox{#1}\vrule}\hrule}}
\let\PsfiG\psfig
\let\PsdrafT\psdraft
\let\PsfulL\psfull
\def\psfig#1{\BoxiT{\PsfiG{#1}}}
\def\BoxiT{\relax}
\def\psdraft{\def\BoxiT{\boxit}\PsdrafT}
\def\psfull{\def\BoxiT{\relax}\PsfulL}

% Attributes of captions below figures and tables.
\newdimen\captionoffset \captionoffset=.5truein  % left offset of captions.
\newdimen\captionwidth \captionwidth=5truein     % width of captions
\newdimen\captionsize \captionsize=5.5truein     % sum of the above
\newdimen\captionspacing \captionspacing=17pt    % baselineskip

\newcount\fignumber \fignumber=0
\def\figdir{.}
\let\figinsert=\topinsert
\def\figheading{}
\def\figurehead#1{\gdef\figheading{#1}}

\def\Figure#1#2#3#4#5\par{
   \assignfigno{#1}
   \let\figinsert=\pageinsert      % temporarily use pageinsert
   \figinsert
   \centerline{\psfig{figure=\figdir/#1,height=#3,width=#4}}
   \bigskip
   \bigskip
   \hsize \captionsize
   \leftskip \captionoffset
   \baselineskip=\captionspacing
   \centerline{\hskip 5em \titlefont #5}
   \nopagenumbers
   \vfil
   \endinsert
}

\def\FigureIgnoreHeight#1#2#3#4#5\par{
   \assignfigno{#1}
   \let\figinsert=\pageinsert      % temporarily use pageinsert
   \figinsert
   \centerline{\psfig{figure=\figdir/#1,width=#4}}
   \bigskip
   \bigskip
   \hsize \captionsize
   \leftskip \captionoffset
   \baselineskip=\captionspacing
   \centerline{\hskip 5em \titlefont #5}
   \nopagenumbers
   \vfil
   \endinsert
}

\def\Figuremid#1#2#3#4#5\par{
   \let\figinsert=\pageinsert      % temporarily use pageinsert
   \Figure{#1}{#2}{#3}{#4}{#5}\par    % do the figure
}

\def\Figurepage#1#2#3#4#5\par{
   \let\figinsert=\pageinsert      % temporarily use pageinsert
   \Figure{#1}{#2}{#3}{#4}{#5}\par    % do the figure
}

\def\FigureComposite#1#2#3#4#5\par{
   \let\figinsert=#3
   \assignfigno{#1}
   \figinsert
   #4
   \bigskip
   \bigskip
   \hsize \captionsize
   \leftskip \captionoffset
   \baselineskip=\captionspacing
   \centerline{\hskip 5em \titlefont #5}
   \nopagenumbers
   \vfil
   \endinsert
}

\def\Figno#1{\assignfigno{#1}\csname figurenumber!#1\endcsname}
\def\Fig#1{Fig.~\Figno{#1}}

\def\assignfigno#1{%
   \expandafter\ifx\csname figurenumber!#1\endcsname\relax%
      \global\advance\fignumber by 1%
      \expandafter\xdef\csname figurenumber!#1\endcsname%
               {\figheading\the\fignumber}%
   \fi%
}

%-------------------------------------------------------------------------

\newcount\chapnumber \chapnumber=0

%\def\chapterskipamount{.23}
\def\chaptertitle#1\par{
   \advance\chapnumber by 1
   \vfill\supereject
%  \chapterstart
   \taghead{\the\chapnumber.}
   \figurehead{}
  \noindent
  \hangindent=1.0truecm \hangafter=1
% {\titlefont \the\chapnumber \hskip 2em #1}
  {\titlefont #1}
  \nobreak\smallskip\noindent
}

\def\sectionskipamount{.15}
\def\acknowledgements\par{
%  \chapterstart
  \bigskip \bigskip
  \vskip0pt plus \sectionskipamount\vsize
  \penalty-250
  \vskip0pt plus-\sectionskipamount\vsize
  \bigskip\vskip\parskip
% \leftline{\sectionfont#1}
  \noindent
  \hangindent=1.0truecm \hangafter=1
  {\titlefont ACKNOWLEDGEMENTS}
  \nobreak\smallskip\noindent
}

\def\appendix#1#2\par{
   \vfill\supereject
%  \chapterstart
   \taghead{#1}
   \figurehead{}
  \noindent
  \hangindent=1.0truecm \hangafter=1
  {\titlefont APPENDIX #1 #2}
  \nobreak\smallskip\noindent
}

\outer\def\beginsection#1\par{
  \bigskip \bigskip
  \vskip0pt plus \sectionskipamount\vsize
  \penalty-250
  \vskip0pt plus-\sectionskipamount\vsize
  \bigskip\vskip\parskip
% \leftline{\sectionfont#1}
  \noindent
  \hangindent=1.0truecm \hangafter=1
  {\sectionfont#1}
  \nobreak\smallskip\noindent}

\outer\def\beginsubsection#1\par{
  \bigskip\bigskip
  \vskip0pt plus \sectionskipamount\vsize
  \penalty-250
  \vskip0pt plus-\sectionskipamount\vsize
  \vskip\parskip
% \leftline{\bf#1}
  \noindent
  \hangindent=1.0truecm \hangafter=1
  {\bf#1}
  \nobreak\smallskip\noindent}


\let\jnlreferences\references
\def\references{
   \vfill\supereject
   \jnlreferences
   \centerline{\titlefont References}
   \bigskip\medskip
}
\let\jnlendreferences\endreferences
\def\endreferences{\jnlendreferences\vfil\eject}


\catcode`@=11
\newcount\r@fcount \r@fcount=0
\newcount\r@fcurr
\immediate\newwrite\reffile
\newif\ifr@ffile\r@ffilefalse
\def\w@rnwrite#1{\ifr@ffile\immediate\write\reffile{#1}\fi\message{#1}}

\def\writer@f#1>>{}
\def\referencefile{%			  Stuff to write .REF file
  \r@ffiletrue\immediate\openout\reffile=\jobname.ref%
  \def\writer@f##1>>{\ifr@ffile\immediate\write\reffile%
    {\noexpand\refis{##1} = \csname r@fnum##1\endcsname = %
     \expandafter\expandafter\expandafter\strip@t\expandafter%
     \meaning\csname r@ftext\csname r@fnum##1\endcsname\endcsname}\fi}%
  \def\strip@t##1>>{}}
\let\referencelist=\referencefile

\def\citeall#1{\xdef#1##1{#1{\noexpand\cite{##1}}}}
\def\cite#1{\each@rg\citer@nge{#1}}   % Variable No. of args, separated by ","

\def\each@rg#1#2{{\let\thecsname=#1\expandafter\first@rg#2,\end,}}
\def\first@rg#1,{\thecsname{#1}\apply@rg}	% each@ag is a general purpose
\def\apply@rg#1,{\ifx\end#1\let\next=\relax%	  variable no. of arg. macro.
\else,\thecsname{#1}\let\next=\apply@rg\fi\next}% args separated by commas

\def\citer@nge#1{\citedor@nge#1-\end-}	% Check for M-N range (M and N numbers)
\def\citer@ngeat#1\end-{#1}
\def\citedor@nge#1-#2-{\ifx\end#2\r@featspace#1 % Single argument
  \else\citel@@p{#1}{#2}\citer@ngeat\fi}	% M-N range of arguments
\def\citel@@p#1#2{\ifnum#1>#2{\errmessage{Reference range #1-#2\space is bad.}
    \errhelp{If you cite a series of references by the notation M-N, then M and
    N must be integers, and N must be greater than or equal to M.}}\else%
 {\count0=#1\count1=#2\advance\count1 by1\relax\expandafter\r@fcite\the\count0,
  \loop\advance\count0 by1\relax%	  Loop from M to N
    \ifnum\count0<\count1,\expandafter\r@fcite\the\count0,%
  \repeat}\fi}

\def\r@featspace#1#2 {\r@fcite#1#2,}	% Eat spaces at beginning or end of arg
\def\r@fcite#1,{\ifuncit@d{#1}		% Cite individual reference
    \expandafter\gdef\csname r@ftext\number\r@fcount\endcsname%
    {\message{Reference #1 to be supplied.}\writer@f#1>>#1 to be supplied.\par
     }\fi%
  \csname r@fnum#1\endcsname}

\def\ifuncit@d#1{\expandafter\ifx\csname r@fnum#1\endcsname\relax%
\global\advance\r@fcount by1%
\expandafter\xdef\csname r@fnum#1\endcsname{\number\r@fcount}}

\let\r@fis=\refis			% Save old \refis, redefine
\def\refis#1#2#3\par{\ifuncit@d{#1}%      Use two params #2 #3 to strip blank
    \w@rnwrite{Reference #1=\number\r@fcount\space is not cited up to now.}\fi%
  \expandafter\gdef\csname r@ftext\csname r@fnum#1\endcsname\endcsname%
  {\writer@f#1>>#2#3\par}}

\def\r@ferr{\endreferences\errmessage{I was expecting to see
\noexpand\endreferences before now;  I have inserted it here.}}
\let\r@ferences=\references
\def\references{\r@ferences\def\endmode{\r@ferr\par\endgroup}}

\let\endr@ferences=\endreferences
\def\endreferences{\r@fcurr=0%		  Save old \endreferences, redefine
  {\loop\ifnum\r@fcurr<\r@fcount%	  Loop over refnum and produce text
    \advance\r@fcurr by 1\relax\expandafter\r@fis\expandafter{\number\r@fcurr}%
    \csname r@ftext\number\r@fcurr\endcsname%
  \repeat}\gdef\r@ferr{}\endr@ferences}

% Save old \endpaper, redefine it to write parting message.

\let\r@fend=\endpaper\gdef\endpaper{\ifr@ffile
\immediate\write16{Cross References written on []\jobname.REF.}\fi\r@fend}

\catcode`@=12

\citeall\refto		% These macros will generate citations
\citeall\ref		%
\citeall\Ref		%


\catcode`@=11
\newcount\tagnumber\tagnumber=0

\immediate\newwrite\eqnfile
\newif\if@qnfile\@qnfilefalse
\def\write@qn#1{}
\def\writenew@qn#1{}
\def\w@rnwrite#1{\write@qn{#1}\message{#1}}
\def\@rrwrite#1{\write@qn{#1}\errmessage{#1}}

\def\taghead#1{\gdef\t@ghead{#1}\global\tagnumber=0}
\def\t@ghead{}

\expandafter\def\csname @qnnum-3\endcsname
  {{\t@ghead\advance\tagnumber by -3\relax\number\tagnumber}}
\expandafter\def\csname @qnnum-2\endcsname
  {{\t@ghead\advance\tagnumber by -2\relax\number\tagnumber}}
\expandafter\def\csname @qnnum-1\endcsname
  {{\t@ghead\advance\tagnumber by -1\relax\number\tagnumber}}
\expandafter\def\csname @qnnum0\endcsname
  {\t@ghead\number\tagnumber}
\expandafter\def\csname @qnnum+1\endcsname
  {{\t@ghead\advance\tagnumber by 1\relax\number\tagnumber}}
\expandafter\def\csname @qnnum+2\endcsname
  {{\t@ghead\advance\tagnumber by 2\relax\number\tagnumber}}
\expandafter\def\csname @qnnum+3\endcsname
  {{\t@ghead\advance\tagnumber by 3\relax\number\tagnumber}}

\def\equationfile{%
  \@qnfiletrue\immediate\openout\eqnfile=\jobname.eqn%
  \def\write@qn##1{\if@qnfile\immediate\write\eqnfile{##1}\fi}
  \def\writenew@qn##1{\if@qnfile\immediate\write\eqnfile
    {\noexpand\tag{##1} = (\t@ghead\number\tagnumber)}\fi}
}

\def\callall#1{\xdef#1##1{#1{\noexpand\call{##1}}}}
\def\call#1{\each@rg\callr@nge{#1}}

\def\each@rg#1#2{{\let\thecsname=#1\expandafter\first@rg#2,\end,}}
\def\first@rg#1,{\thecsname{#1}\apply@rg}
\def\apply@rg#1,{\ifx\end#1\let\next=\relax%
\else,\thecsname{#1}\let\next=\apply@rg\fi\next}

\def\callr@nge#1{\calldor@nge#1-\end-}
\def\callr@ngeat#1\end-{#1}
\def\calldor@nge#1-#2-{\ifx\end#2\@qneatspace#1 %
  \else\calll@@p{#1}{#2}\callr@ngeat\fi}
\def\calll@@p#1#2{\ifnum#1>#2{\@rrwrite{Equation range #1-#2\space is bad.}
\errhelp{If you call a series of equations by the notation M-N, then M and
N must be integers, and N must be greater than or equal to M.}}\else%
 {\count0=#1\count1=#2\advance\count1 by1\relax\expandafter\@qncall\the\count0,
  \loop\advance\count0 by1\relax%
    \ifnum\count0<\count1,\expandafter\@qncall\the\count0,%
  \repeat}\fi}

\def\@qneatspace#1#2 {\@qncall#1#2,}
\def\@qncall#1,{\ifunc@lled{#1}{\def\next{#1}\ifx\next\empty\else
  \w@rnwrite{Equation number \noexpand\(>>#1<<) has not been defined yet.}
  >>#1<<\fi}\else\csname @qnnum#1\endcsname\fi}

\let\eqnono=\eqno
\def\eqno(#1){\tag#1}
\def\tag#1$${\eqnono(\displayt@g#1 )$$}

\def\aligntag#1\endaligntag
  $${\gdef\tag##1\\{&(##1 )\cr}\eqalignno{#1\\}$$
  \gdef\tag##1$${\eqnono(\displayt@g##1 )$$}}

\let\eqalignnono=\eqalignno

\def\eqalignno#1{\displ@y \tabskip\centering
  \halign to\displaywidth{\hfil$\displaystyle{##}$\tabskip\z@skip
    &$\displaystyle{{}##}$\hfil\tabskip\centering
    &\llap{$\displayt@gpar##$}\tabskip\z@skip\crcr
    #1\crcr}}

\def\displayt@gpar(#1){(\displayt@g#1 )}

\def\displayt@g#1 {\rm\ifunc@lled{#1}\global\advance\tagnumber by1
        {\def\next{#1}\ifx\next\empty\else\expandafter
        \xdef\csname @qnnum#1\endcsname{\t@ghead\number\tagnumber}\fi}%
  \writenew@qn{#1}\t@ghead\number\tagnumber\else
        {\edef\next{\t@ghead\number\tagnumber}%
        \expandafter\ifx\csname @qnnum#1\endcsname\next\else
        \w@rnwrite{Equation \noexpand\tag{#1} is a duplicate number.}\fi}%
  \csname @qnnum#1\endcsname\fi}

\def\ifunc@lled#1{\expandafter\ifx\csname @qnnum#1\endcsname\relax}

\let\@qnend=\end\gdef\end{\if@qnfile
\immediate\write16{Equation numbers written on []\jobname.EQN.}\fi\@qnend}

\catcode`@=12


